Htex: Per-Halfedge Texturing for Arbitrary Mesh Topologies

We introduce per-halfedge texturing (Htex) a GPU-friendly method for texturing arbitrary polygon-meshes without an explicit parameterization. Htex builds upon the insight that halfedges encode an intrinsic triangulation for polygon meshes, where each halfedge spans a unique triangle with direct adjacency information. Rather than storing a separate texture per face of the input mesh as is done by previous parameterization-free texturing methods, Htex stores a square texture for each halfedge and its twin. We show that this simple change from face to halfedge induces two important properties for high performance parameterization-free texturing. First, Htex natively supports arbitrary polygons without requiring dedicated code for, e.g, non-quad faces. Second, Htex leads to a straightforward and efficient GPU implementation that uses only three texture-fetches per halfedge to produce continuous texturing across the entire mesh. We demonstrate the effectiveness of Htex by rendering production assets in real time.

==> figures/figure-halfedge-mesh.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.097365, 0.857855) -- (-0.580000, 0.480000) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.400291, 0.279877) {\scalebox{0.729000}{$f_{0}$}};
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.208751, 0.159164) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (-0.225627, -0.215749) {\scalebox{0.729000}{$f_{1}$}};
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.530444, 0.655336) -- cycle;
\node[mygrey, draw = none, anchor = center]
at (0.240842, 0.221945) {\scalebox{0.729000}{$f_{2}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.338682, 0.668927) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.338682, 0.668927) {\scalebox{0.729000}{$e_{0}$}};
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.647524, 0.051244) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.647524, 0.051244) {\scalebox{0.729000}{$e_{1}$}};
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.234065, -0.433205) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.234065, -0.433205) {\scalebox{0.729000}{$e_{2}$}};
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.461899, -0.109174) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.461899, -0.109174) {\scalebox{0.729000}{$e_{3}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.208751, 0.159164);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.153058, 0.508509) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.153058, 0.508509) {\scalebox{0.729000}{$e_{4}$}};
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.019084, -0.164867) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.019084, -0.164867) {\scalebox{0.729000}{$e_{5}$}};
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.489941, -0.281315) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.489941, -0.281315) {\scalebox{0.729000}{$e_{6}$}};
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.631704, 0.290801) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.631704, 0.290801) {\scalebox{0.729000}{$e_{7}$}};
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.216540, 0.756595) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.216540, 0.756595) {\scalebox{0.729000}{$e_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.584357, -0.117574) -- (-0.293236, 0.191014);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.438796, 0.036720) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.438796, 0.036720) {\scalebox{0.729000}{$h_{0}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.277794, 0.221898) -- (-0.213747, 0.623646);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.245770, 0.422772) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.245770, 0.422772) {\scalebox{0.729000}{$h_{1}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.223028, 0.631667) -- (-0.500543, 0.414400);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.361786, 0.523033) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.361786, 0.523033) {\scalebox{0.729000}{$h_{2}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.515985, 0.383516) -- (-0.593638, -0.109554);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.554812, 0.136981) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.554812, 0.136981) {\scalebox{0.729000}{$h_{3}$}};
\draw[myorange, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.000000]}]
(-0.507466, -0.327135) -- (0.045664, -0.381182);
\draw[myorange, fill = myorangelighter, line width = 0.8]
(-0.230901, -0.34) circle (0.06);
\node[myorange, draw = none, anchor = center]
at (-0.230901, -0.34) {\scalebox{0.8}{$h_{4}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.058322, -0.377765) -- (-0.203688, -0.005130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.072683, -0.191448) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.072683, -0.191448) {\scalebox{0.729000}{$h_{5}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.227737, -0.002345) -- (-0.518858, -0.310934);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.373297, -0.156640) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.373297, -0.156640) {\scalebox{0.729000}{$h_{6}$}};
\draw[myblue, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.000000]}]
(0.026678, 0.601921) -- (-0.037369, 0.200174);
\draw[myblue, fill = mybluelighter, line width = 0.8000]
(-0.005345, 0.401048) circle (0.06000);
\node[myblue, draw = none, anchor = center]
at (-0.005345, 0.401048) {\scalebox{0.8}{$h_{7}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.028762, 0.166505) -- (0.233248, -0.206130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.102243, -0.019813) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.102243, -0.019813) {\scalebox{0.729000}{$h_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.256790, -0.211953) -- (0.536267, 0.026767);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.396529, -0.092593) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.396529, -0.092593) {\scalebox{0.729000}{$h_{9}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.543355, 0.055373) -- (0.426906, 0.474587);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.485131, 0.264980) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.485131, 0.264980) {\scalebox{0.729000}{$h_{10}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.406148, 0.497877) -- (0.045158, 0.614326);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.225653, 0.556101) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.225653, 0.556101) {\scalebox{0.729000}{$h_{11}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.580000, 0.480000) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.580000, 0.480000) {\scalebox{0.729000}{$v_{0}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.097365, 0.857855) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.097365, 0.857855) {\scalebox{0.729000}{$v_{1}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.208751, 0.159164) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.208751, 0.159164) {\scalebox{0.729000}{$v_{2}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.715048, -0.377512) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.715048, -0.377512) {\scalebox{0.729000}{$v_{3}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.246918, -0.488898) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.246918, -0.488898) {\scalebox{0.729000}{$v_{4}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.732964, -0.073733) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.732964, -0.073733) {\scalebox{0.729000}{$v_{5}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.530444, 0.655336) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.530444, 0.655336) {\scalebox{0.729000}{$v_{6}$}};

==> figures/figure-htex-halfedges.tex <==
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.208751, 0.159164) -- (-0.097365, 0.857855) -- (-0.580000, 0.480000) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (0.246918, -0.488898) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.208751, 0.159164) -- (0.246918, -0.488898) -- (0.732964, -0.073733) -- (0.530444, 0.655336) -- cycle;
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.584357, -0.117574) -- (-0.293236, 0.191014);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.438796, 0.036720) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.438796, 0.036720) {\scalebox{0.729000}{$h_{0}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.277794, 0.221898) -- (-0.213747, 0.623646);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.245770, 0.422772) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.245770, 0.422772) {\scalebox{0.729000}{$h_{1}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.223028, 0.631667) -- (-0.500543, 0.414400);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.361786, 0.523033) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.361786, 0.523033) {\scalebox{0.729000}{$h_{2}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.515985, 0.383516) -- (-0.593638, -0.109554);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.554812, 0.136981) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.554812, 0.136981) {\scalebox{0.729000}{$h_{3}$}};
\draw[myorange, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.500000]}]
(-0.507466, -0.327135) -- (0.045664, -0.391182);
\draw[myorange, fill = myorangelighter, line width = 0.8]
(-0.230901, -0.359159) circle (0.1);
\node[myorange, draw = none, anchor = center]
at (-0.230901, -0.359159) {\scalebox{0.8}{$h_{4}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.058322, -0.377765) -- (-0.203688, -0.005130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.072683, -0.191448) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.072683, -0.191448) {\scalebox{0.729000}{$h_{5}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.227737, -0.002345) -- (-0.518858, -0.310934);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.373297, -0.156640) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (-0.373297, -0.156640) {\scalebox{0.729000}{$h_{6}$}};
\draw[myblue, line width = 0.8, ->, > = stealth, -{Latex[length = 4.000000, width = 4.500000]}]
(0.026678, 0.601921) -- (-0.037369, 0.200174);
\draw[myblue, fill = mybluelighter, line width = 0.8000]
(-0.005345, 0.401048) circle (0.1);
\node[myblue, draw = none, anchor = center]
at (-0.005345, 0.401048) {\scalebox{0.8}{$h_{7}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(-0.028762, 0.166505) -- (0.233248, -0.206130);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.102243, -0.019813) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (0.102243, -0.019813) {\scalebox{0.729000}{$h_{8}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.256790, -0.211953) -- (0.536267, 0.026767);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.396529, -0.092593) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (0.396529, -0.092593) {\scalebox{0.729000}{$h_{9}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.543355, 0.055373) -- (0.426906, 0.474587);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.485131, 0.264980) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (0.485131, 0.264980) {\scalebox{0.729000}{$h_{10}$}};
\draw[mygrey, line width = 0.075000, ->, > = stealth, -{Latex[length = 3.000000, width = 3.000000]}]
(0.406148, 0.497877) -- (0.045158, 0.614326);
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.225653, 0.556101) circle (0.081000);
\node[mygrey, draw = none, anchor = center]
at (0.225653, 0.556101) {\scalebox{0.729000}{$h_{11}$}};

==> figures/figure-htex-parameterization-detail.tex <==
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.715048, -0.377512) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.400291, 0.279877) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.400291, 0.279877) -- (-0.097365, 0.857855) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.400291, 0.279877) -- (-0.580000, 0.480000) -- cycle;
\fill[mygreylighter]
(0.246918, -0.488898) -- (-0.225627, -0.235749) -- (-0.715048, -0.377512) -- cycle;
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.225627, -0.235749) -- (0.246918, -0.488898) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.225627, -0.235749) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(-0.208751, 0.159164) -- (0.240842, 0.221945) -- (-0.097365, 0.857855) -- cycle;
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.240842, 0.221945) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.240842, 0.221945) -- (0.246918, -0.488898) -- cycle;
\fill[mygreylighter]
(0.530444, 0.655336) -- (0.240842, 0.221945) -- (0.732964, -0.073733) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (0.240842, 0.221945) -- (0.530444, 0.655336) -- cycle;
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (0.240842, 0.221945);

\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
%\draw[mygrey, line width = 0.600000]
%(-0.208751, 0.159164) -- (-0.715048, -0.377512);
%\draw[mygrey, line width = 0.600000]
%(-0.097365, 0.857855) -- (-0.208751, 0.159164);
%\draw[mygrey, line width = 0.600000]
%(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);

\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.338682, 0.668927) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.338682, 0.668927) {\scalebox{0.729000}{$q_{0}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.647524, 0.051244) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.647524, 0.051244) {\scalebox{0.729000}{$q_{1}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(-0.234065, -0.433205) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.234065, -0.433205) {\scalebox{0.729000}{$q_{2}$}};
%\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
%(-0.461899, -0.109174) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.461899, -0.109174) {\scalebox{0.729000}{$q_{3}$}};
%\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
%(-0.153058, 0.508509) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (-0.153058, 0.508509) {\scalebox{0.729000}{$q_{4}$}};
%\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
%(0.019084, -0.164867) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.019084, -0.164867) {\scalebox{0.729000}{$q_{5}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.489941, -0.281315) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.489941, -0.281315) {\scalebox{0.729000}{$q_{6}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.631704, 0.290801) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.631704, 0.290801) {\scalebox{0.729000}{$q_{7}$}};
\draw[mygreylighter, fill = mygreylight, line width = 0.075000]
(0.216540, 0.756595) circle (0.045000);
\node[mygrey, draw = none, anchor = center]
at (0.216540, 0.756595) {\scalebox{0.729000}{$q_{8}$}};

==> figures/figure-htex-parameterization.tex <==
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (0.240842, 0.221945);

\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
%\draw[mygrey, line width = 0.600000]
%(-0.208751, 0.159164) -- (-0.715048, -0.377512);
%\draw[mygrey, line width = 0.600000]
%(-0.097365, 0.857855) -- (-0.208751, 0.159164);
%\draw[mygrey, line width = 0.600000]
%(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);

==> figures/figure-htex-rendering.tex <==
\draw[mygreylighter, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\draw[mygreylighter, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.400291, 0.279877);
\draw[mygreylighter, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.400291, 0.279877);
\draw[mygreylighter, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\draw[mygreylighter, line width = 0.600000]
(0.246918, -0.488898) -- (-0.225627, -0.235749);
\draw[mygreylighter, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.225627, -0.235749);
\draw[mygreylighter, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\draw[mygreylighter, line width = 0.600000]
(-0.208751, 0.159164) -- (0.240842, 0.221945);
\draw[mygreylighter, line width = 0.600000]
(0.246918, -0.488898) -- (0.240842, 0.221945);
\draw[mygreylighter, line width = 0.600000]
(0.732964, -0.073733) -- (0.240842, 0.221945);
\draw[mygreylighter, line width = 0.600000]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\draw[mygreylighter, line width = 0.600000]
(-0.097365, 0.857855) -- (0.240842, 0.221945);

\draw[mygreylighter, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygreylighter, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[mygreylighter, line width = 0.600000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygreylighter, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygreylighter, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygreylighter, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);

==> figures/figure-htex-triangulation.tex <==
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.400291, 0.279877) -- (-0.715048, -0.377512) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (-0.400291, 0.279877) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(-0.580000, 0.480000) -- (-0.400291, 0.279877) -- (-0.097365, 0.857855) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.400291, 0.279877) -- (-0.580000, 0.480000) -- cycle;
\fill[myorangelighter]
(0.246918, -0.488898) -- (-0.225627, -0.235749) -- (-0.715048, -0.377512) -- cycle;
\fill[mygreylighter]
(-0.208751, 0.159164) -- (-0.225627, -0.235749) -- (0.246918, -0.488898) -- cycle;
\fill[mygreylighter]
(-0.715048, -0.377512) -- (-0.225627, -0.235749) -- (-0.208751, 0.159164) -- cycle;
\fill[mybluelighter]
(-0.208751, 0.159164) -- (0.240842, 0.221945) -- (-0.097365, 0.857855) -- cycle;
\fill[mygreylighter]
(0.246918, -0.488898) -- (0.240842, 0.221945) -- (-0.208751, 0.159164) -- cycle;
\fill[mygreylighter]
(0.732964, -0.073733) -- (0.240842, 0.221945) -- (0.246918, -0.488898) -- cycle;
\fill[mygreylighter]
(0.530444, 0.655336) -- (0.240842, 0.221945) -- (0.732964, -0.073733) -- cycle;
\fill[mygreylighter]
(-0.097365, 0.857855) -- (0.240842, 0.221945) -- (0.530444, 0.655336) -- cycle;
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.400291, 0.279877);
\node[mygrey, draw = none, anchor = center]
at (-0.441363, 0.020509) {\scalebox{0.729000}{$t_{0}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.400291, 0.279877);
\node[mygrey, draw = none, anchor = center]
at (-0.235469, 0.432298) {\scalebox{0.729000}{$t_{1}$}};
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.400291, 0.279877);
\node[mygrey, draw = none, anchor = center]
at (-0.359219, 0.539244) {\scalebox{0.729000}{$t_{2}$}};
\draw[mygrey, line width = 0.600000]
(-0.715048, -0.377512) -- (-0.400291, 0.279877);
\node[mygrey, draw = none, anchor = center]
at (-0.565113, 0.127455) {\scalebox{0.729000}{$t_{3}$}};
\draw[myorange, line width = 0.800000]
(0.246918, -0.488898) -- (-0.225627, -0.235749);
\node[myorange, draw = none, anchor = center]
at (-0.231253, -0.337386) {\scalebox{0.9}{$t_{4}$}};
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.225627, -0.235749);
\node[mygrey, draw = none, anchor = center]
at (-0.062487, -0.188494) {\scalebox{0.729000}{$t_{5}$}};
\draw[myorange, line width = 0.800000]
(-0.715048, -0.377512) -- (-0.225627, -0.235749);
\node[mygrey, draw = none, anchor = center]
at (-0.383142, -0.151366) {\scalebox{0.729000}{$t_{6}$}};
\draw[myblue, line width = 0.800000]
(-0.208751, 0.159164) -- (0.240842, 0.221945);
\node[myblue, draw = none, anchor = center]
at (-0.021758, 0.412988) {\scalebox{0.9}{$t_{7}$}};
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.240842, 0.221945);
\node[mygrey, draw = none, anchor = center]
at (0.093003, -0.035930) {\scalebox{0.729000}{$t_{8}$}};
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.240842, 0.221945);
\node[mygrey, draw = none, anchor = center]
at (0.406908, -0.113562) {\scalebox{0.729000}{$t_{9}$}};
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (0.240842, 0.221945);
\node[mygrey, draw = none, anchor = center]
at (0.501417, 0.267849) {\scalebox{0.729000}{$t_{10}$}};
\draw[myblue, line width = 0.800000]
(-0.097365, 0.857855) -- (0.240842, 0.221945);
\node[mygrey, draw = none, anchor = center]
at (0.224640, 0.578378) {\scalebox{0.729000}{$t_{11}$}};
\draw[mygrey, line width = 0.600000]
(-0.097365, 0.857855) -- (-0.580000, 0.480000);
\draw[mygrey, line width = 0.600000]
(-0.580000, 0.480000) -- (-0.715048, -0.377512);
\draw[myorange, line width = 0.800000]
(-0.715048, -0.377512) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (-0.715048, -0.377512);
\draw[myblue, line width = 0.800000]
(-0.097365, 0.857855) -- (-0.208751, 0.159164);
\draw[mygrey, line width = 0.600000]
(-0.208751, 0.159164) -- (0.246918, -0.488898);
\draw[mygrey, line width = 0.600000]
(0.246918, -0.488898) -- (0.732964, -0.073733);
\draw[mygrey, line width = 0.600000]
(0.732964, -0.073733) -- (0.530444, 0.655336);
\draw[mygrey, line width = 0.600000]
(0.530444, 0.655336) -- (-0.097365, 0.857855);
